Two-particle azimuthal correlations as a probe of collective behaviour in deep inelastic $\textit{ep}$ scattering at HERA

Two-particle azimuthal correlations have been measured in neutral current deep $\mbox{inelastic}$ $\textit{ep}$ scattering with virtuality $Q^2 > 5$ GeV$^2$ at a centre-of-mass energy $\sqrt{s}=318$ GeV recorded with the ZEUS detector at HERA. The correlations of charged particles have been measured in the range of laboratory pseudorapidity $-1.5 < \eta < 2.0$ and transverse momentum $0.1 < p_{\textrm{T}}~< 5.0$ GeV and event multiplicities $N_{\textrm{ch}}$ up to six times larger than the average $\left< N_{\textrm{ch}} \right>\approx5$. The two-particle correlations have been measured in terms of the angular observables $c_n\{2\}=\left< \left< \cos{ n \Delta\varphi} \right> \right>$, where $n$ is between 1 and 4 and $\Delta\varphi$ is the relative azimuthal angle between the two particles. Comparisons with available models of deep inelastic scattering, which are tuned to reproduce inclusive particle production, suggest that the measured two-particle correlations are dominated by contributions from multijet production. The correlations observed here do not indicate the kind of collective behaviour recently observed at the highest RHIC and LHC energies in high-multiplicity hadronic collisions.

==> auth187_new.tex <==
     





%===================================================================
%
%  MEMBER NAME  AUTH183 (ZEUS)     M  TEX
%
%  JH.: transformed to a format, which is suited as input for
%       CONVERT, which automatically creates author-indices
%
%  Don't remove lines starting with a percent sign %,
%  CONVERT may need them urgently !
%  
%=====================================================================

                                                   %
\begin{center}
{                      \Large  The ZEUS Collaboration              }
\end{center}

{\small\raggedright


%  members:

I.~Abt$^{19}$, 
L.~Adamczyk$^{7}$, 
R. Aggarwal$^{3, b}$, 
V.~Aushev$^{17}$, 
O.~Behnke$^{9}$, 
U.~Behrens$^{9}$, 
A.~Bertolin$^{21}$, 
I.~Bloch$^{10}$, 
I.~Brock$^{2}$, 
N.H.~Brook$^{28, m}$, 
R.~Brugnera$^{22}$, 
A.~Bruni$^{1}$, 
P.J.~Bussey$^{11}$, 
A.~Caldwell$^{19}$, 
M.~Capua$^{4}$, 
C.D.~Catterall$^{32}$, 
J.~Chwastowski$^{6}$, 
J.~Ciborowski$^{29, o}$, 
R.~Ciesielski$^{9, d}$, 
A.M.~Cooper-Sarkar$^{20}$, 
M.~Corradi$^{1, a}$, 
R.K.~Dementiev$^{18}$, 
S.~Dusini$^{21}$, 
J.~Ferrando$^{9}$, 
S.~Floerchinger$^{33}$,
B.~Foster$^{20, j}$, 
E.~Gallo$^{13, k}$, 
D.~Gangadharan$^{14}$, 
A.~Garfagnini$^{22}$, 
A.~Geiser$^{9}$, 
L.K.~Gladilin$^{18}$, 
Yu.A.~Golubkov$^{18}$, 
G.~Grzelak$^{29}$, 
C.~Gwenlan$^{20}$, 
D.~Hochman$^{31}$, 
N.Z.~Jomhari$^{9}$, 
I.~Kadenko$^{17}$, 
S.~Kananov$^{23}$, 
U.~Karshon$^{31}$, 
P.~Kaur$^{3, c}$, 
R.~Klanner$^{13}$, 
U.~Klein$^{9, e}$, 
I.A.~Korzhavina$^{18}$, 
N.~Kovalchuk$^{13}$, 
H.~Kowalski$^{9}$, 
O.~Kuprash$^{9, f}$, 
M.~Kuze$^{25}$, 
B.B.~Levchenko$^{18}$, 
A.~Levy$^{23}$, 
B.~L\"ohr$^{9}$, 
E.~Lohrmann$^{13}$, 
A.~Longhin$^{22}$, 
O.Yu.~Lukina$^{18}$, 
I.~Makarenko$^{9}$, 
J.~Malka$^{9, g}$, 
S.~Masciocchi$^{12, i}$, 
K.~Nagano$^{15}$, 
J.D.~Nam$^{24}$, 
J.~Onderwaater$^{14, l}$, 
Yu.~Onishchuk$^{17}$, 
E.~Paul$^{2}$, 
I.~Pidhurskyi$^{17}$, 
A.~Polini$^{1}$, 
M.~Przybycie\'n$^{7}$, 
A.~Quintero$^{24}$, 
M.~Ruspa$^{27}$, 
D.H.~Saxon$^{11}$, 
U.~Schneekloth$^{9}$, 
T.~Sch\"orner-Sadenius$^{9}$, 
I.~Selyuzhenkov$^{12}$, 
M.~Shchedrolosiev$^{17}$, 
L.M.~Shcheglova$^{18}$, 
I.O.~Skillicorn$^{11}$, 
W.~S{\l}omi\'nski$^{8}$, 
A.~Solano$^{26}$, 
L.~Stanco$^{21}$, 
N.~Stefaniuk$^{9}$, 
P.~Stopa$^{6}$, 
B.~Surrow$^{24}$, 
J.~Sztuk-Dambietz$^{13, g}$, 
E.~Tassi$^{4}$, 
K.~Tokushuku$^{15}$, 
M.~Turcato$^{13, g}$, 
O.~Turkot$^{9}$, 
T.~Tymieniecka$^{30}$, 
A.~Verbytskyi$^{19}$, 
W.A.T.~Wan Abdullah$^{5}$, 
K.~Wichmann$^{9}$, 
M.~Wing$^{28, n}$, 
S.~Yamada$^{15}$, 
Y.~Yamazaki$^{16}$, 
A.F.~\.Zarnecki$^{29}$, 
L.~Zawiejski$^{6}$, 
O.~Zenaiev$^{9, h}$ 
\newpage

%       institutes:

{\setlength{\parskip}{0.4em}
\makebox[3ex]{$^{1}$}
\begin{minipage}[t]{14cm}
{\it INFN Bologna, Bologna, Italy}~$^{A}$

\end{minipage}

\makebox[3ex]{$^{2}$}
\begin{minipage}[t]{14cm}
{\it Physikalisches Institut der Universit\"at Bonn,
Bonn, Germany}~$^{B}$

\end{minipage}

\makebox[3ex]{$^{3}$}
\begin{minipage}[t]{14cm}
{\it Panjab University, Department of Physics, Chandigarh, India}

\end{minipage}

\makebox[3ex]{$^{4}$}
\begin{minipage}[t]{14cm}
{\it Calabria University,
Physics Department and INFN, Cosenza, Italy}~$^{A}$

\end{minipage}

\makebox[3ex]{$^{5}$}
\begin{minipage}[t]{14cm}
{\it National Centre for Particle Physics, Universiti Malaya, 50603 Kuala Lumpur, Malaysia}~$^{C}$

\end{minipage}

\makebox[3ex]{$^{6}$}
\begin{minipage}[t]{14cm}
{\it The Henryk Niewodniczanski Institute of Nuclear Physics, Polish Academy of \\
Sciences, Krakow, Poland}

\end{minipage}

\makebox[3ex]{$^{7}$}
\begin{minipage}[t]{14cm}
{\it AGH University of Science and Technology, Faculty of Physics and Applied Computer
Science, Krakow, Poland}

\end{minipage}

\makebox[3ex]{$^{8}$}
\begin{minipage}[t]{14cm}
{\it Department of Physics, Jagellonian University, Krakow, Poland}~$^{D}$

\end{minipage}

\makebox[3ex]{$^{9}$}
\begin{minipage}[t]{14cm}
{\it Deutsches Elektronen-Synchrotron DESY, Hamburg, Germany}

\end{minipage}

\makebox[3ex]{$^{10}$}
\begin{minipage}[t]{14cm}
{\it Deutsches Elektronen-Synchrotron DESY, Zeuthen, Germany}

\end{minipage}

\makebox[3ex]{$^{11}$}
\begin{minipage}[t]{14cm}
{\it School of Physics and Astronomy, University of Glasgow,
Glasgow, United Kingdom}~$^{E}$

\end{minipage}

\makebox[3ex]{$^{12}$}
\begin{minipage}[t]{14cm}
{\it GSI Helmholtzzentrum f\"{u}r Schwerionenforschung GmbH, Darmstadt, Germany}~$^{K}$

\end{minipage}

\makebox[3ex]{$^{13}$}
\begin{minipage}[t]{14cm}
{\it Hamburg University, Institute of Experimental Physics, Hamburg,
Germany}~$^{F}$

\end{minipage}

\makebox[3ex]{$^{14}$}
\begin{minipage}[t]{14cm}
{\it Physikalisches Institute, University of Heidelberg, Heidelberg, Germany~$^{K}$}

\end{minipage}

\makebox[3ex]{$^{15}$}
\begin{minipage}[t]{14cm}
{\it Institute of Particle and Nuclear Studies, KEK,
Tsukuba, Japan}~$^{G}$

\end{minipage}

\makebox[3ex]{$^{16}$}
\begin{minipage}[t]{14cm}
{\it Department of Physics, Kobe University, Kobe, Japan}~$^{G}$

\end{minipage}

\makebox[3ex]{$^{17}$}
\begin{minipage}[t]{14cm}
{\it Department of Nuclear Physics, National Taras Shevchenko University of Kyiv, Kyiv, Ukraine}

\end{minipage}

\makebox[3ex]{$^{18}$}
\begin{minipage}[t]{14cm}
{\it Lomonosov Moscow State University, Skobeltsyn Institute of Nuclear Physics,
Moscow, Russia}

\end{minipage}

\makebox[3ex]{$^{19}$}
\begin{minipage}[t]{14cm}
{\it Max-Planck-Institut f\"ur Physik, M\"unchen, Germany}

\end{minipage}

\makebox[3ex]{$^{20}$}
\begin{minipage}[t]{14cm}
{\it Department of Physics, University of Oxford,
Oxford, United Kingdom}~$^{E}$

\end{minipage}

\makebox[3ex]{$^{21}$}
\begin{minipage}[t]{14cm}
{\it INFN Padova, Padova, Italy}~$^{A}$

\end{minipage}

\makebox[3ex]{$^{22}$}
\begin{minipage}[t]{14cm}
{\it Dipartimento di Fisica e Astronomia dell' Universit\`a and INFN,
Padova, Italy}~$^{A}$

\end{minipage}

\makebox[3ex]{$^{23}$}
\begin{minipage}[t]{14cm}
{\it Raymond and Beverly Sackler Faculty of Exact Sciences, School of Physics, \\
Tel Aviv University, Tel Aviv, Israel}~$^{H}$

\end{minipage}

\makebox[3ex]{$^{24}$}
\begin{minipage}[t]{14cm}
{\it Department of Physics, Temple University, Philadelphia, PA 19122, USA}~$^{I}$

\end{minipage}

\makebox[3ex]{$^{25}$}
\begin{minipage}[t]{14cm}
{\it Department of Physics, Tokyo Institute of Technology,
Tokyo, Japan}~$^{G}$

\end{minipage}

\makebox[3ex]{$^{26}$}
\begin{minipage}[t]{14cm}
{\it Universit\`a di Torino and INFN, Torino, Italy}~$^{A}$

\end{minipage}

\makebox[3ex]{$^{27}$}
\begin{minipage}[t]{14cm}
{\it Universit\`a del Piemonte Orientale, Novara, and INFN, Torino,
Italy}~$^{A}$

\end{minipage}

\makebox[3ex]{$^{28}$}
\begin{minipage}[t]{14cm}
{\it Physics and Astronomy Department, University College London,
London, United Kingdom}~$^{E}$

\end{minipage}

\makebox[3ex]{$^{29}$}
\begin{minipage}[t]{14cm}
{\it Faculty of Physics, University of Warsaw, Warsaw, Poland}

\end{minipage}

\makebox[3ex]{$^{30}$}
\begin{minipage}[t]{14cm}
{\it National Centre for Nuclear Research, Warsaw, Poland}

\end{minipage}

\makebox[3ex]{$^{31}$}
\begin{minipage}[t]{14cm}
{\it Department of Particle Physics and Astrophysics, Weizmann
Institute, Rehovot, Israel}

\end{minipage}

\makebox[3ex]{$^{32}$}
\begin{minipage}[t]{14cm}
{\it Department of Physics, York University, Ontario, Canada M3J 1P3}~$^{J}$

\end{minipage}

\makebox[3ex]{$^{33}$}
\begin{minipage}[t]{14cm}
{\it Institute for Theoretical Physics, University of Heidelberg, Heidelberg, Germany~$^{K}$}

\end{minipage}

}
\vspace{3em}

%  references concerning institutes;

{\setlength{\parskip}{0.4em}\raggedright
\makebox[3ex]{$^{ A}$}
\begin{minipage}[t]{14cm}
 supported by the Italian National Institute for Nuclear Physics (INFN) \
\end{minipage}

\makebox[3ex]{$^{ B}$}
\begin{minipage}[t]{14cm}
 supported by the German Federal Ministry for Education and Research (BMBF), under
 contract No.\ 05 H09PDF\
\end{minipage}

\makebox[3ex]{$^{ C}$}
\begin{minipage}[t]{14cm}
 supported by HIR grant UM.C/625/1/HIR/149 and UMRG grants RU006-2013, RP012A-13AFR and RP012B-13AFR from
 Universiti Malaya, and ERGS grant ER004-2012A from the Ministry of Education, Malaysia\
\end{minipage}

\makebox[3ex]{$^{ D}$}
\begin{minipage}[t]{14cm}
supported by the Polish National Science Centre (NCN) grant no.\ DEC-2014/13/B/ST2/02486
\end{minipage}

\makebox[3ex]{$^{ E}$}
\begin{minipage}[t]{14cm}
 supported by the Science and Technology Facilities Council, UK\
\end{minipage}

\makebox[3ex]{$^{ F}$}
\begin{minipage}[t]{14cm}
 supported by the German Federal Ministry for Education and Research (BMBF), under
 contract No.\ 05h09GUF, and the SFB 676 of the Deutsche Forschungsgemeinschaft (DFG) \
\end{minipage}

\makebox[3ex]{$^{ G}$}
\begin{minipage}[t]{14cm}
 supported by the Japanese Ministry of Education, Culture, Sports, Science and Technology
 (MEXT) and its grants for Scientific Research\
\end{minipage}

\makebox[3ex]{$^{ H}$}
\begin{minipage}[t]{14cm}
 supported by the Israel Science Foundation\
\end{minipage}

\makebox[3ex]{$^{ I}$}
\begin{minipage}[t]{14cm}
 supported in part by the Office of Nuclear Physics within the U.S.\ DOE Office of Science
\end{minipage}

\makebox[3ex]{$^{ J}$}
\begin{minipage}[t]{14cm}
 supported by the Natural Sciences and Engineering Research Council of Canada (NSERC) \
\end{minipage}

\makebox[3ex]{$^{ K}$}
\begin{minipage}[t]{14cm}
this work is part of and supported by the DFG Collaborative Research 
Centre ``SFB 1225 (ISOQUANT)''\
\end{minipage}


}

\pagebreak[4]
{\setlength{\parskip}{0.4em}

%  references concerning members;

\makebox[3ex]{$^{ a}$}
\begin{minipage}[t]{14cm}
now at INFN Roma, Italy\
\end{minipage}

\makebox[3ex]{$^{ b}$}
\begin{minipage}[t]{14cm}
now at DST-Inspire Faculty, Department of Technology, SPPU, India\
\end{minipage}

\makebox[3ex]{$^{ c}$}
\begin{minipage}[t]{14cm}
now at Sant Longowal Institute of Engineering and Technology, Longowal, Punjab, India\
\end{minipage}

\makebox[3ex]{$^{ d}$}
\begin{minipage}[t]{14cm}
now at Rockefeller University, New York, NY 10065, USA\
\end{minipage}

\makebox[3ex]{$^{ e}$}
\begin{minipage}[t]{14cm}
now at University of Liverpool, United Kingdom\
\end{minipage}

\makebox[3ex]{$^{ f}$}
\begin{minipage}[t]{14cm}
now at University of Freiburg, Freiburg, Germany\
\end{minipage}

\makebox[3ex]{$^{ g}$}
\begin{minipage}[t]{14cm}
now at European X-ray Free-Electron Laser facility GmbH, Hamburg, Germany\
\end{minipage}

\makebox[3ex]{$^{ h}$}
\begin{minipage}[t]{14cm}
now at Hamburg University, Hamburg, Germany\
\end{minipage}

\makebox[3ex]{$^{ i}$}
\begin{minipage}[t]{14cm}
also at Physikalisches Institut of the University of Heidelberg, Heidelberg,  Germany\
\end{minipage}

\makebox[3ex]{$^{ j}$}
\begin{minipage}[t]{14cm}
also at DESY and University of Hamburg\
\end{minipage}

\makebox[3ex]{$^{ k}$}
\begin{minipage}[t]{14cm}
also at DESY\
\end{minipage}

\makebox[3ex]{$^{ l}$}
\begin{minipage}[t]{14cm}
also at GSI Helmholtzzentrum f\"{u}r Schwerionenforschung GmbH, Darmstadt, Germany\
\end{minipage}

\makebox[3ex]{$^{ m}$}
\begin{minipage}[t]{14cm}
now at University of Bath, United Kingdom\
\end{minipage}

\makebox[3ex]{$^{ n}$}
\begin{minipage}[t]{14cm}
also supported by DESY\
\end{minipage}

\makebox[3ex]{$^{ o}$}
\begin{minipage}[t]{14cm}
also at Lodz University, Poland\
\end{minipage}

}


}


